FPRF: Feed-Forward Photorealistic Style Transfer of Large-Scale 3D Neural Radiance Fields

We present FPRF, a feed-forward photorealistic style transfer method for large-scale 3D neural radiance fields. FPRF stylizes large-scale 3D scenes with arbitrary, multiple style reference images without additional optimization while preserving multi-view appearance consistency. Prior arts required tedious per-style/-scene optimization and were limited to small-scale 3D scenes. FPRF efficiently stylizes large-scale 3D scenes by introducing a style-decomposed 3D neural radiance field, which inherits AdaIN's feed-forward stylization machinery, supporting arbitrary style reference images. Furthermore, FPRF supports multi-reference stylization with the semantic correspondence matching and local AdaIN, which adds diverse user control for 3D scene styles. FPRF also preserves multi-view consistency by applying semantic matching and style transfer processes directly onto queried features in 3D space. In experiments, we demonstrate that FPRF achieves favorable photorealistic quality 3D scene stylization for large-scale scenes with diverse reference images. Project page: https://kim-geonu.github.io/FPRF/

==> figures/LLFF_comparison.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/LLFF_comparison/LLFF_comparison_v2.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{(Will write soon) Using the trim and clip commands produces fragile layers that can result in disasters }
    \label{fig:LLFF_comparison}
\end{figure*}

==> figures/large_scale_comparison.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/large_scale_comparison/large_scale_comparison_v4.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{(Will write soon) Using the trim and clip commands produces fragile layers that can result in disasters }
    \label{fig:large_scale_comparison}
\end{figure*}

==> figures/prop_table.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/prop_table/prop_table_v2.pdf}
    \caption{\textbf{\emph{UrbanStyle} properties.} \emph{UrbanStyle} provides a photorealistic, feed-forward style transfer method for large-scale neural radiance fields, while supporting multiple style reference images in the stylization stage. \emph{UrbanStyle} differs from competing methods, where it needs only a single training stage, and it works with arbitrary style images.}
    \label{tab:property}
\end{figure}


==> figures/rebuttal_dino12.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]    {figures/rebuttal_dino12/dino12.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    % \vspace{-6mm}
    \caption{Comparison of stylization results with DINO v2
    }
    \label{fig:rebuttal_dino12}
\end{figure}

==> figures/rebuttal_vgg.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/rebuttal_vgg/vgg_3.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \vspace{-7mm}
    \caption{
    {
    Ablation study for VGG feature distillation loss \(\mathcal{L}_{\text{VGG}}\) on the LLFF dataset.
    }
    }\vspace{-5mm}
    \label{fig:rebuttal_vgg}
\end{figure}

==> figures/scene_reconstruction.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/scene_reconstruction/scene_reconstruction.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{\textbf{Comparison with the baseline model.}
    We compare rendering quality of UrbanStyle with the baseline model on the LLFF~\cite{mildenhall2019local} dataset.
    The baseline denotes a model has same architecture with UrbanStyle, but is trained with learnable decoder from scratch.
    UrbanStyle shows comparable results with the baseline.}
    \label{table: scene reconstruction}
\end{figure}

	

==> figures/semantic_ablation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/semantic_ablation/semantic_ablation_v2.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{\textbf{Global-local style trade-off.}
    The first column shows the original scene and the reference image, and others show the stylized scene according to the global style code's blending ratio \(\alpha\). Semantic-aware local AdaIN allows us to avoid global style transfer, which often produces unsatisfactory results, especially for large-scale scenes containing diverse components.}
    % \vspace{-0.3cm}
    \label{fig:semantic_ablation_method}
\end{figure}

==> tables/consistency.tex <==
\begin{table}[t]
		\small
		\setlength\tabcolsep{1.5pt}
            \renewcommand{\arraystretch}{1.2}
		\begin{tabular}{l|cccccccc|c}
			\toprule
                % \hline
			& fern & flower & fortress & horns & leaves & orchids & room & trex & Avg. \\ 
   % \cmidrule{1-10}
   \hline
			$\text{MKL}$&   \textbf{29.38}   &    33.70  & \textbf{36.05}  &  31.92  &    27.91   &    28.01    &   32.75   &    30.79  &   31.31  \\ 
   \hline
			UPST&     &      &       &      &       &     &    &    &   \\  
			% \cmidrule{1-10}
   \hline
			Ours &  29.29   &   \textbf{33.75}    &    34.44     &  \textbf{32.37}   &   \textbf{29.72}    &    \textbf{29.75}     &  \textbf{33.67}   &   \textbf{31.10}   &   \textbf{31.76}  \\ 	
   % \hline
   \bottomrule
   \toprule
    % \cmidrule{1-10}
	% \cmidrule{1-10}		
			% \hline
			$\text{MKL}$&  \textbf{24.77}   &  \textbf{28.60}   &    \textbf{29.54}    &    \textbf{28.54}   &    24.52    &   22.95    &   27.73   &  26.45    &  26.64 \\ 
   \hline
			UPST&  &     &       &     &      &        &     &     &  \\   
			\hline
                % \cmidrule{1-10}
			Ours &   24.39   &   27.97    &     27.47     &   28.50   &    \textbf{26.41}   &   \textbf{24.19}   &  \textbf{28.31}   &  \textbf{26.72}   &   \textbf{26.75}  \\ 	
                \bottomrule

		\end{tabular}
		\vspace{-0.3cm}
		\caption{Comparisons of short (upper) and long  (lower) temporary consistency on LLFF dataset.}
		\label{table: short temporary}
		\vspace{-1em}
	\end{table}

==> tables/rebuttal_consistency.tex <==
\begin{table}[t]
\centering
    % \setlength
    % \tabcolsep{11.5pt}
        % \renewcommand{\arraystretch}{1.2}
    % \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l cccc}
        \toprule
        & {CCPL} & {\(\text{PhotoWCT}^2\)} & {UPST} &  {Ours}\\
        % & Photorealistic & FF & TT & MS\\

        \midrule

        % training
        PSNR (long)  ($\uparrow$) &  19.98 & \underline{20.94} & - & \textbf{22.38} \\
        % PSNR (long)  (\uparrow) &  19.98 & \underline{20.94} & - & \textbf{22.38} \\

        PSNR (short) ($\uparrow$) &  24.61 & \underline{27.64} & - & \textbf{29.71} \\

        \midrule
        \midrule

        % training
        PSNR (long) ($\uparrow$) &  24.14 & 26.81 & \textbf{28.16} & \underline{28.06} \\

        PSNR (short) ($\uparrow$) &  26.44 & 32.29 & \textbf{33.00} & \underline{32.78} \\


        \bottomrule
    \end{tabular}
    }
    \caption{Comparisons of multi-view consistency on the San Francisco Mission Bay dataset (upper) and the LLFF dataset (lower).
    }
    \vspace{-3mm}
    \label{tab:rebuttal_consistency}
\end{table}


==> tables/rebuttal_sifid_lpips.tex <==
\begin{table}[t]
\centering
    % \setlength
    % \tabcolsep{11.5pt}
        % \renewcommand{\arraystretch}{1.2}
    % \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l cccc}
        \toprule
        & {CCPL} & {{PhotoWCT}\textsuperscript{2}} & {UPST} &  {Ours}\\
        % & Photorealistic & FF & TT & MS\\

        \midrule
        San Francisco Mission Bay 
        \midrule

        % training
        LPIPS ($\downarrow$) &  0.48 & \underline{0.34} & - & \textbf{0.32} \\

        SIFID ($\downarrow$) &  \textbf{1.08} & \underline{1.31} & - & 1.37 \\

        \midrule
        \midrule

        % training
        LPIPS ($\downarrow$) &  0.42 & \underline{0.30} & 0.33 & \textbf{0.30} \\

        SIFID ($\downarrow$) &  \textbf{1.13} & 1.40 & 1.83 & \underline{1.31} \\


        \bottomrule
    \end{tabular}
    }
    \caption{Comparisons of photorealistic style transfer quality on the San Francisco Mission Bay dataset (upper) and the LLFF dataset (lower).
    }
    \vspace{-2mm}
    \label{tab:rebuttal_sifid_lpips}
\end{table}


==> tables/rebuttal_unified.tex <==
\begin{table}[t]
% \centering
    % \setlength
    % \tabcolsep{11.5pt}
        % \renewcommand{\arraystretch}{1.2}
    {
    % \footnotesize
    \scriptsize
    \renewcommand{\arraystretch}{0.7}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l cccc}
        \toprule
        & {CCPL} & {{PhotoWCT}\textsuperscript{2}} & {UPST-NeRF} &  {Ours}\\
        % & Photorealistic & FF & TT & MS\\

        \midrule
        \multicolumn{5}{c}{San Francisco Mission Bay dataset} \\
        \midrule

        % training
        LPIPS ($\downarrow$) &  0.48 & \underline{0.34} & - & \textbf{0.32} \\

        SIFID ($\downarrow$) &  \textbf{1.08} & \underline{1.31} & - & 1.37 \\

        PSNR (long)  ($\uparrow$) &  19.98 & \underline{20.94} & - & \textbf{22.38} \\
        % PSNR (long)  (\uparrow) &  19.98 & \underline{20.94} & - & \textbf{22.38} \\

        PSNR (short) ($\uparrow$) &  24.61 & \underline{27.64} & - & \textbf{29.71} \\

        \midrule
        \midrule
        \multicolumn{5}{c}{LLFF dataset} \\
        \midrule

        % training
        LPIPS ($\downarrow$) &  0.42 & \underline{0.30} & 0.33 & \textbf{0.30} \\

        SIFID ($\downarrow$) &  \textbf{1.13} & 1.40 & 1.83 & \underline{1.31} \\

        PSNR (long) ($\uparrow$) &  24.14 & 26.81 & \textbf{28.16} & \underline{28.06} \\

        PSNR (short) ($\uparrow$) &  26.44 & 32.29 & \textbf{33.00} & \underline{32.78} \\


        \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
    % Comparisons of 
    % photorealistic style transfer quality and multi-view consistency 
    % on the San Francisco Mission Bay dataset (upper) and the LLFF dataset (lower). 
    {Comparisons of
    % We compare 
    the PST quality (LPIPS, SIFID) and the multi-view consistency (PSNRs).
    % of different methods 
    % on the San Francisco Mission Bay dataset (upper) and the LLFF dataset (lower).
    }
    % 
    % {We use 16 style images from the PST dataset~[C4], 160 content images from each large-scale and small-scale dataset for comparison.}
    % asd
    }
    \vspace{-2mm}
    % \vspace{0mm}
    % 
    \label{tab:rebuttal_unified}
    }
\end{table}




